Sublinear Algorithms for Gap Edit Distance

The edit distance is a way of quantifying how similar two strings are to one another by counting the minimum number of character insertions, deletions, and substitutions required to transform one string into the other. A simple dynamic programming computes the edit distance between two strings of length $n$ in $O(n^2)$ time, and a more sophisticated algorithm runs in time $O(n+t^2)$ when the edit distance is $t$ [Landau, Myers and Schmidt, SICOMP 1998]. In pursuit of obtaining faster running time, the last couple of decades have seen a flurry of research on approximating edit distance, including polylogarithmic approximation in near-linear time [Andoni, Krauthgamer and Onak, FOCS 2010], and a constant-factor approximation in subquadratic time [Chakrabarty, Das, Goldenberg, Kouck\'y and Saks, FOCS 2018]. We study sublinear-time algorithms for small edit distance, which was investigated extensively because of its numerous applications. Our main result is an algorithm for distinguishing whether the edit distance is at most $t$ or at least $t^2$ (the quadratic gap problem) in time $\tilde{O}(\frac{n}{t}+t^3)$. This time bound is sublinear roughly for all $t$ in $[\omega(1), o(n^{1/3})]$, which was not known before. The best previous algorithms solve this problem in sublinear time only for $t=\omega(n^{1/3})$ [Andoni and Onak, STOC 2009]. Our algorithm is based on a new approach that adaptively switches between uniform sampling and reading contiguous blocks of the input strings. In contrast, all previous algorithms choose which coordinates to query non-adaptively. Moreover, it can be extended to solve the $t$ vs $t^{2-\epsilon}$ gap problem in time $\tilde{O}(\frac{n}{t^{1-\epsilon}}+t^3)$.

==> fig_block.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=.7,shorten >=.65mm,>=latex]
 \tikzstyle gridlines=[color=black!20,very thin]
 \draw[color=black!20,very thin] (0,0) grid (8,8);

 \foreach \x in {0,...,8}
  \foreach \y in {0,...,8}
   {
     \draw[fill,color=black!50] (\x,\y) circle (0.65mm);
     %\draw[->,dashed,thick] (\x,\y)--(\x+1,\y);
     %\draw[->,dashed,thick] (\x,\y+1)--(\x,\y);
   }
   \foreach \x in {0,...,7}
  \foreach \y in {1,...,8}
   {
     \draw[->,dashed,thick] (\x,\y)--(\x+1,\y);
     \draw[->,dashed,thick] (\x,\y)--(\x,\y-1);
     \draw[->,dashed,thick] (\x,\y)--(\x+1,\y-1);
   }
   \foreach \y in {1,...,8}
   {
     \draw[->,dashed,thick] (0,\y)--(0,\y-1);
     \draw[->,dashed,thick] (8,\y)--(8,\y-1);
   }
   \foreach \x in {0,...,7}
   {
     \draw[->,dashed,thick] (\x,0)--(\x+1,0);
     \draw[->,dashed,thick] (\x,8)--(\x+1,8);
   }

 %\draw[step=1cm,color=black!30,very thin] (0,-.25) grid (8.25,1.25);

 %\tikzstyle{every node}=[draw,shape=circle,fill=red!20]
 
 
%  \draw[very thin,fill=white!70!gray] (1,0) rectangle (2,1);
  \draw[fill=white!70!gray] (0,8) rectangle (5,5);
  \draw[fill=white!70!gray] (0,6) rectangle (7,3);
  \draw[fill=white!70!gray] (2,4) rectangle (8,1);
  \draw[fill=white!70!gray] (4,2) rectangle (8,0);
  \draw[-,dashed,thick] (0,5)--(5,5);
  \draw[-,dashed,thick] (5,6)--(5,5);
  \draw[-,dashed,thick] (2,3)--(7,3);
  \draw[-,dashed,thick] (7,4)--(7,3);
  \draw[-,dashed,thick] (4,1)--(8,1);
  \draw[-,>=latex,thick] (0,6)--(6,0);
  \draw[-,>=latex,thick] (2,8)--(8,2);
  \draw[-,>=latex,thick] (0,8)--(8,0);
  %\draw[-,>=latex,thick] (0,7)--(7,0);
  %\draw[-,>=latex,thick] (1,8)--(8,1);
  \node at (2,4.5) {$-k$};
  \node at (4,4.5) {$0$};
  \node at (6,4.5) {$k$};
  %\draw[fill,color=black] (4,4) circle (0.65mm);
  %\draw[fill,color=black] (4,6) circle (0.65mm);
  %\draw[fill,color=black] (2,4) circle (0.65mm);


  
  %\node at (1,7) {$G_1$};
  %\node at (5,3) {$G_2$};
  %\draw[-,dashed,thick] (4,4)--(4,5);
  %\node at (3.7,4.5) {$L_v(2,2)$};
  %\draw[-,dashed,thick] (4,4)--(5,4);
  %\node at (4.5,3.5) {$L_h(2,2)$};
  

\end{tikzpicture}
\caption{Sketch of a block-wise division of edit graph.}
   \label{fig:block}
\end{figure}


==> fig_edit.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=1.5,shorten >=1mm,>=latex]
 \tikzstyle gridlines=[color=black!20,very thin]
 %old scoring scheme
 \draw[color=black!20,very thin] (0,0) grid (3,3);

 \foreach \x in {0,...,3}
  \foreach \y in {0,...,3}
   {
     \draw[fill,color=black!50] (\x,\y) circle (0.65mm);
   }
 \foreach \x in {0,...,2}
  \foreach \y in {1,...,3}
   {
     \draw[->,dashed,thick] (\x,\y)--(\x+1,\y);
     \draw[->,dashed,thick] (\x,\y)--(\x,\y-1);
     \draw[->,dashed,thick] (\x,\y)--(\x+1,\y-1);
   }
   \foreach \y in {1,...,3}
   {
     \draw[->,dashed,thick] (0,\y)--(0,\y-1);
     \draw[->,dashed,thick] (3,\y)--(3,\y-1);
     \node at (0.5,\y-0.1) {$1$};
     \node at (1.5,\y-0.1) {$1$};
     \node at (2.5,\y-0.1) {$1$};
   }
   \foreach \x in {0,...,2}
   {
     \draw[->,dashed,thick] (\x,0)--(\x+1,0);
     \draw[->,dashed,thick] (\x,3)--(\x+1,3);
     \node at (\x+0.1,2.5) {$1$};
     \node at (\x+0.1,1.5) {$1$};
     \node at (\x+0.1,0.5) {$1$};
   }
   %string x
   \node at (-0.5,3) {$x$};
   \node at (-0.5,0.5) {$A$};
   \node at (-0.5,1.5) {$B$};
   \node at (-0.5,2.5) {$A$};
   %string y
   \node at (-0.5,3.5) {$y$};
   \node at (0.5,3.5) {$A$};
   \node at (1.5,3.5) {$A$};
   \node at (2.5,3.5) {$B$};
   %cost function
   \node at (0.6,2.6) {$0$};
   \node at (1.6,2.6) {$0$};
   \node at (2.6,2.6) {$1$};
   \node at (0.6,1.6) {$1$};
   \node at (1.6,1.6) {$1$};
   \node at (2.6,1.6) {$0$};
   \node at (0.6,0.6) {$0$};
   \node at (1.6,0.6) {$0$};
   \node at (2.6,0.6) {$1$};
   \node at (0.5,-0.1) {$1$};
   \node at (1.5,-0.1) {$1$};
   \node at (2.5,-0.1) {$1$};
   \node at (3.1,2.5) {$1$};
   \node at (3.1,1.5) {$1$};
   \node at (3.1,0.5) {$1$};
   \node at (-0.2,3.2) {$(0,0)$};
   \node at (3.2,-0.2) {$(3,3)$};
%    \node at (1.5,-1) {(a) standard scoring scheme};
% 
%  %new scoring scheme
%  \draw[color=black!20,very thin] (5,0) grid (8,3);
% 
%  \foreach \x in {5,...,8}
%   \foreach \y in {0,...,3}
%    {
%      \draw[fill,color=black!50] (\x,\y) circle (0.65mm);
%    }
%  \foreach \x in {5,...,7}
%   \foreach \y in {1,...,3}
%    {
%      \draw[->,dashed,thick] (\x,\y)--(\x+1,\y);
%      \draw[->,dashed,thick] (\x,\y)--(\x,\y-1);
%      \draw[->,dashed,thick] (\x,\y)--(\x+1,\y-1);
%    }
%    \foreach \y in {1,...,3}
%    {
%      \draw[->,dashed,thick] (5,\y)--(5,\y-1);
%      \draw[->,dashed,thick] (8,\y)--(8,\y-1);
%      
%    }
%    \foreach \x in {5,...,7}
%    {
%      \draw[->,dashed,thick] (\x,0)--(\x+1,0);
%      \draw[->,dashed,thick] (\x,3)--(\x+1,3);
%      \node at (\x+0.5,2.9) {$2$};
%      \node at (\x+0.1,0.5) {$2$};
%    }
%    %string x
%    \node at (4.5,3) {$x$};
%    \node at (4.5,0.5) {$A$};
%    \node at (4.5,1.5) {$B$};
%    \node at (4.5,2.5) {$A$};
%    %string y
%    \node at (4.5,3.5) {$y$};
%    \node at (5.5,3.5) {$A$};
%    \node at (6.5,3.5) {$A$};
%    \node at (7.5,3.5) {$B$};
%    %cost function
%    \node at (5.6,2.6) {$0$};
%    \node at (6.6,2.6) {$0$};
%    \node at (7.6,2.6) {$1$};
%    \node at (5.6,1.6) {$1$};
%    \node at (6.6,1.6) {$1$};
%    \node at (7.6,1.6) {$0$};
%    \node at (5.6,0.6) {$0$};
%    \node at (6.6,0.6) {$0$};
%    \node at (7.6,0.6) {$1$};
%    \node at (5.5,-0.1) {$0$};
%    \node at (6.5,-0.1) {$0$};
%    \node at (7.5,-0.1) {$0$};
%    \node at (8.1,2.5) {$0$};
%    \node at (8.1,1.5) {$0$};
%    \node at (8.1,0.5) {$0$};
%    \node at (5.5,0.9) {$0$};
%    \node at (6.5,0.9) {$0$};
%    \node at (7.5,0.9) {$2$};
%    \node at (5.5,1.9) {$0$};
%    \node at (6.5,1.9) {$2$};
%    \node at (7.5,1.9) {$2$};
%    \node at (6.1,2.5) {$0$};
%    \node at (7.1,2.5) {$0$};
%    \node at (7.1,1.5) {$0$};
%    \node at (6.1,1.5) {$2$};
%    \node at (5.1,0.5) {$2$};
%    \node at (5.1,1.5) {$2$};
%    \node at (5.1,2.5) {$2$};
%    \node at (4.8,3.2) {$(0,0)$};
%    \node at (8.2,-0.2) {$(3,3)$};
%    \node at (6.5,-1) {(b) new scoring scheme};
%  
% 

\end{tikzpicture}
\caption{An example of edit graph for string $x,y \in \{A,B\}^3$}
   \label{fig:editgraph}
   
\end{figure}

==> mature_diag.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.3,shorten >=1mm,>=latex]
 \tikzstyle gridlines=[color=black!20,very thin]
 %old scoring scheme
% \draw[color=black!20,very thin] (0,0) grid (20,20);

% \foreach \x in {0,...,3}
%  \foreach \y in {0,...,3}
%   {
%     \draw[fill,color=black!50] (\x,\y) circle (0.65mm);
%   }
\draw[color=black!20,thin] (-1,9) rectangle (18,21);
%\draw[rectangle](21,0)--(15,11);



\draw[-,thick](0,20)--(2,18);
\draw[-,dashed](2,18)--(10,10);
\draw[fill,color=gray!50] (10,10) circle (2mm);

\draw[-,thick](1,20)--(4,17);
\draw[-,dashed](4,17)--(11,10);
\draw[fill,color=gray!50] (11,10) circle (2mm);


\draw[-,thick](3,20)--(4,19);
\draw[fill,color=gray!50] (4,19) circle (2mm);

\draw[-,thick](4,20)--(15,10);
\draw[fill,color=gray!50] (15,10) circle (2mm);
%\draw[fill,color=gray!50] (1,19) circle (2mm);
%\draw[-,thick](1,19)--(3,17);

%
%\draw[fill,color=gray!50] (1,18) circle (2mm);
%\draw[-,thick](1,18)--(5,14);
%\draw[-,dashed,thick](1,18)--(9,10);
%\draw[-,thick](1,20)--(5,16);
%\draw[-,dashed,thick](5,16)--(11,10);
%\draw[-,thick](5,20)--(10,15);
%\draw[-,dashed,thick](10,15)--(15,10);
%\draw[-,thick](6,20)--(7,19);
%\draw[fill,color=gray!50] (8,19) circle (2mm);
%\draw[-,thick](8,19)--(17,10);
%\draw[fill,color=gray!50] (7,19) circle (2mm);
%\draw[-,thick](7,19)--(9,17);
%\draw[fill,color=gray!50] (9,17) circle (2mm);
%
%\draw[fill,color=gray!50] (9,10) circle (2mm);
%\draw[fill,color=gray!50] (11,10) circle (2mm);
%\draw[fill,color=gray!50] (15,10) circle (2mm);




% \foreach \x in {0,2,5}
%  \foreach \y in {0,...,19}
%   {
%     \draw[-,thick] (\x,\y)--(\x-1,\y-1);
%%     \draw[-,dashed,thick] (\x,\y)--(\x,\y-1);
%%     \draw[-,dashed,thick] (\x,\y)--(\x+1,\y-1);
%   }
%   \node at (-0.5,20.5) {$-4$};
%   
%   \node at (0.5,20.5) {$-3$};
%   \foreach \y in {1,...,3}
%   {
%     \draw[->,dashed,thick] (0,\y)--(0,\y-1);
%     \draw[->,dashed,thick] (3,\y)--(3,\y-1);
%     \node at (0.5,\y-0.1) {$1$};
%     \node at (1.5,\y-0.1) {$1$};
%     \node at (2.5,\y-0.1) {$1$};
%   }
%   \foreach \x in {0,...,2}
%   {
%     \draw[->,dashed,thick] (\x,0)--(\x+1,0);
%     \draw[->,dashed,thick] (\x,3)--(\x+1,3);
%     \node at (\x+0.1,2.5) {$1$};
%     \node at (\x+0.1,1.5) {$1$};
%     \node at (\x+0.1,0.5) {$1$};
%   }
%   %cost function
%   \node at (0.6,2.6) {$0$};
%   \node at (1.6,2.6) {$0$};
%   \node at (2.6,2.6) {$1$};
%   \node at (0.6,1.6) {$1$};
%   \node at (1.6,1.6) {$1$};
%   \node at (2.6,1.6) {$0$};
%   \node at (0.6,0.6) {$0$};
%   \node at (1.6,0.6) {$0$};
%   \node at (2.6,0.6) {$1$};
%   \node at (0.5,-0.1) {$1$};
%   \node at (1.5,-0.1) {$1$};
%   \node at (2.5,-0.1) {$1$};
%   \node at (3.1,2.5) {$1$};
%   \node at (3.1,1.5) {$1$};
%   \node at (3.1,0.5) {$1$};
%   \node at (-0.2,3.2) {$(0,0)$};
%   \node at (3.2,-0.2) {$(3,3)$};

\end{tikzpicture}
\caption{Illustration of the slides performed by Algorithm~\ref{alg:noSuffixTree}: Diagonals on which the algorithm compares character by character are marked by continuous lines; Mature diagonals which are not the right most are marked by dashed lines;  Edit operations are marked by a circle.}
   \label{fig:matureDiag}
\end{figure}
